Similarity Driven Approximation for Text Analytics

Text analytics has become an important part of business intelligence as enterprises increasingly seek to extract insights for decision making from text data sets. Processing large text data sets can be computationally expensive, however, especially if it involves sophisticated algorithms. This challenge is exacerbated when it is desirable to run different types of queries against a data set, making it expensive to build multiple indices to speed up query processing. In this paper, we propose and evaluate a framework called EmApprox that uses approximation to speed up the processing of a wide range of queries over large text data sets. The key insight is that different types of queries can be approximated by processing subsets of data that are most similar to the queries. EmApprox builds a general index for a data set by learning a natural language processing model, producing a set of highly compressed vectors representing words and subcollections of documents. Then, at query processing time, EmApprox uses the index to guide sampling of the data set, with the probability of selecting each subcollection of documents being proportional to its {\em similarity} to the query as computed using the vector representations. We have implemented a prototype of EmApprox as an extension of the Apache Spark system, and used it to approximate three types of queries: aggregation, information retrieval, and recommendation. Experimental results show that EmApprox's similarity-guided sampling achieves much better accuracy than random sampling. Further, EmApprox can achieve significant speedups if users can tolerate small amounts of inaccuracies. For example, when sampling at 10\%, EmApprox speeds up a set of queries counting phrase occurrences by almost 10x while achieving estimated relative errors of less than 22\% for 90\% of the queries.

==> background.tex <==
\guangyannote{backup}
\subsection{Cluster sampling}
Online sampling at the cluster level is more efficient for large dataset, since sampling only at the data item level still requires a full scan of the dataset. A cluster sample with equal probabilities over the sampling units may result in a large variance, whereas sampling with unequal inclusion probabilities \textit{probability proportional to size}~(pps), it can decrease variance~\cite{lohr2009sampling}.

In AQP, ``size'' can refer to the amount of relevant data to a specific query in each cluster containing a variety of keys. Intuitively, sampling clusters that have higher probabilities to contain relevant data is a more efficient sampling design. However, the precise size of a cluster is usually unknown until being processed, so auxiliary information of clusters that indicates its relevancy to computation is used to estimate the inclusion probabilities.
\futurenote{
	pps sampling can also have two stages, where data items in the chosen clusters are also sampled with probabilities proportional to their relevancy of a computation.
%\futurenote{Explicit formulas}

Here is an analysis about how pps reduces sampling error compared to simple random sampling~(srs). Both estimators  $\hat{\tau}_{pps}$ and  $\hat{\tau}_{srs}$ are unbiased, so $E[\hat{\tau}_{pps}]$ = $E[\hat{\tau}_{srs}]$ = $\tau$~\cite{lohr2009sampling}: 
\begin{align*}
	\hat{\tau}_{pps} = \frac{1}{n}\sum_{i \in S}\frac{\tau_{i}}{\psi_i}  \quad\text{and}\quad \hat{\tau}_{srs} = \frac{N}{n}\sum_{i \in S} \tau_{i}
\end{align*}
\noindent where $\tau_{i}$ is the sum of the values in cluster $i$, $\psi_{i}$ as the inclusion probability of cluster $i$; $n$ is the number of chosen clusters out of $N$. The variances are:
\begin{align*}
	V_{pps} =\frac{\sum_{i \in S} (\frac{\tau_i}{\psi_i} - \tau)^2}{n(n-1)}\quad\text{and}\quad
	V_{srs} = \frac{(N^2-Nn)s^2_t}{n}
\end{align*}
\noindent where in $V_{srs}$:
\begin{equation*}
	s^2_t = \frac{1}{n-1}\sum_{i \in S}(\tau_i - \tau)^2
\end{equation*}

\subsection{Cluster Sampling - A Primer}
Suppose we want to estimate the frequency $\tau$ of a phrase $Z$ occurring in a large data set partitioned into disjoint subcollections of documents. If we take a cluster sample from the data set using subcollections as the sampling units, we can derive the estimator $\hat{\tau}$ using cluster sampling theory~\cite{lohr2009sampling}:
\begin{align*}
	\hat{\tau} = \frac{1}{n}\sum_{s \in S}\frac{\tau_{s}}{\phi_{s}} \pm \epsilon
\end{align*}
where $S$ is the chosen sample, $s$ is a subcollection in the sample, $\tau_{s}$ is the frequency of the target phrase in subcollection $s$,  $\phi_{s}$ is the sampling probability for $s$,
and $\epsilon$ is the estimated error bounds. $\epsilon$ in turn is computed as:
\begin{align*}
	\epsilon = t_{n-1, 1-\alpha/2} \sqrt{\hat{V} (\hat{\tau})} = t_{n-1, 1-\alpha/2} \sqrt{\frac{\sum_{s \in S} (\frac{\tau_{s}}{\phi_{s}} - \hat{\tau})^2}{n(n-1)}}
\end{align*}
where $n$ is the sample size and $t_{n-1, 1-\alpha/2}$ is the critical value of a $t$-distribution at confidence level $\alpha$ with $n-1$ degrees of freedom. We observe that as the $\phi_{s}$'s approach $\frac{\tau_{s}}{\hat{\tau}}$, $\hat{V} (\hat{\tau})$ and hence $\epsilon$ will approach 0. Thus, using {\it probability proportional to size}~(pps) sampling~\cite{lohr2009sampling}, we can reduce the error bound for our estimator $\hat{\tau}$ by leveraging auxiliary information about the dataset to set each $\phi_{s}$ to be close to $\frac{\tau_{s}}{\hat{\tau}}$. If $\hat{\tau}$ is a good estimator, then $\phi_{s}$ should be close to $\frac{\tau_{s}}{\tau}$, which is proportional to how strongly $s$ ``predicts'' $Z$ in the context of NLP~\cite{lin2015hierarchical}.


We see that when $\psi_{i}$ is approaching $\frac{\tau_{i}}{\tau}$, the value of $V_{pps}$ approaches to zero, whereas for $V_{pps}$ to approach zero, the queried data would have to be distributed evenly across the clusters. The latter case would be rare, however, when we have auxiliary information to estimate the amount of relevant data in each cluster, we will have an estimator coupled with much less uncertainty.}

\subsection{Neural embedding language models} 

Recent advances in Natural Language Processing (NLP) have shown that semantically meaningful representations of words and documents can be efficiently learned by neural embedding models.
A popular unsupervised neural network based language model known as word2vec, learns vector representations for words that encode words' semantic similarities~\cite{word2vec}. A word's similarity with other words can be defined by the context under which the words are usually used. The model's training objective maximizes the joint probability of the words in a text dataset by predicting its context words, and outputs the vector representations of each word. Therefore word similarities can be quantified by computing the dot product based similarity between their vector representations. These learned vectors exhibit additive compositionality, enabling semantic reasoning through simple arithmetics such as element-wise addition over different vectors~\cite{word2vec}. For example, $vec(``king") - vec(``man") \approx vec(``queen") - vec(``woman")$.

In addition to word vectors, vectors for paragraphs and documents can also be learned. Paragraph Vector~(PV) is a model that jointly learns vector representation for words and a piece of variable-length text ranging from sentences to documents, through an unsupervised framework based on word2vec~\cite{doc2vec}. PV-DBOW (Distributed Bag of Words version of Paragraph Vector) is a version of PV that has been shown to be effective in information retrieval~\cite{paragraphVectorIR} due to its direct relationship to word distributions in the text datasets. Training objective of PV-DBOW is similar to word2vec, where it maximizes the joint probability of documents or paragraphs in a corpus by predicting the observed words included in the text. Under PV-DBOW, the probability of word $w$ in document $d$ is modeled using a softmax function:
\begin{equation}
P_{PV}(w|d) = \frac{exp(\vec{w} \cdot \vec{d})}{\sum_{w^\prime \in V_w} exp(\vec{w^\prime} \cdot \vec{d})}
\label{eq:PVSoftmax}
\end{equation}
where $\vec{w}$ and $\vec{d}$ are vector representations for $w$ and $d$, $V_w$ is the vocabulary. To make gradient computation more efficient when $V_w$ is large, a technique called negative sampling was proposed in~\cite{word2vec} to approximate equation~(\ref{eq:PVSoftmax}). It actually changes the training objective by trying to maximize the similarityjoint probability between document $d$ and words $w$ that are included in the document,of the while minimizing the similarity between document $d$ and a ``negative'' word $w_N$ that is not included in the word-document pairs $(w, d)$ within the dataset, while ``negative'' pairs $(w_N, d)$ are not, and both of the probabilities can be computed using the sigmoid function defined as: $\sigma~(\vec{x} \cdot \vec{y}) = 1/(1 + e^{-\vec{x}\cdot\vec{y}})$. The global training objective of PV-DBOW using negative sampling is:
\begin{equation}
l = \sum_{(w,d) \in D}\#(w,d)~(log~\sigma(\vec{w} \cdot \vec{d})~
+ k~\cdot E_{w_N \sim P_{n}}[log~\sigma(-\vec{w_{N}} \cdot \vec{d})])
\label{eq:PVTrainingObj}
\end{equation}
where $\#(w,d)$ denotes the frequency of an observed word-document pair, $D$ is the corpus, $V_D$ is the vocabulary, $k$ is the number of negative samples, $\sigma$ is the sigmoid function and $E_{w_N \sim P_{v}}[log~\sigma(-\vec{w_{N}} \cdot \vec{d})]$ is the expected value of $log~\sigma(-\vec{w_{N}} \cdot \vec{d})$ given a noise distribution $P_{n}$ for $w_N$~\cite{le2014distributed}.

\subsection{Locality-sensitive hashing}
LSH was originally proposed for solving the nearest neighbor~(NN) search problem over high-dimensional large datasets~\cite{ANNLsh, gionis1999similarity}. The basic idea behind LSH is to transform each item in a d-dimensional space into a binary bit vector with $b$ bits, using hash functions $h_0$, ..., $h_b$. Each hash function $h$ must satisfy the property:
\begin{equation*}
	Pr[h(\vec{x}) = h(\vec{y})] = sim(\vec{x}, \vec{y})
\end{equation*}
where $\vec{x}$ and $\vec{y}$ represent the vector representations of two items $x$ and $y$ in the dataset; $sim$ is a similarity measure, including Jaccard, Euclidean, cosine, etc. Similarity between two items is preserved in the mapping, that is, if two items have identical or similar binary bit vectors then the probability that they are close to each other in the original d-dimensional space is also high. \yongfengnote{Since in this work $\vec{x}$ and $\vec{y}$ are real-valued vectors, maybe it is necessary to discuss how LSH is used to encode these real-value vectors}

There are two common ways that LSH bit vectors can index a dataset, depending on whether hash table is involved~\cite{wang2014hashing}. Using a hash table, the dataset can be indexed by storing items with the same bit vectors in the same buckets. As an example, items in the same buckets can be compared with each other using the precise similarity metric to output an approximate set of pair-wised similar items in the dataset, eliminating the need for a full $O(n^2)$ scan. Without using hash table, the bit vectors can be directly used as index to rank items against the query in a faster way albeit approximately, exploiting the property that two bit vectors' distance can be computed very efficiently using exclusive OR. The bit vector based ranking can quickly filter out less relevant items to the query. The latter case is more similar to our proposed approach for indexing the dataset for approximate computations.
